Bounded Context Switching for Valence Systems

We study valence systems, finite-control programs over infinite-state memories modeled in terms of graph monoids. Our contribution is a notion of bounded context switching (BCS). Valence systems generalize pushdowns, concurrent pushdowns, and Petri nets. In these settings, our definition conservatively generalizes existing notions. The main finding is that reachability within a bounded number of context switches is in NP, independent of the memory (the graph monoid). Our proof is genuinely algebraic, and therefore contributes a new way to think about BCS. In addition, we exhibit a class of storage mechanisms for which BCS reachability belongs to P.

==> content/abstract_unused.tex <==

Besides 
that applies to programs working over arbitrary storage structures.
thinking about bounded context switching
The notion solely refer to the memorywith memories moveled inover graph monoids as memories.
The notion is intuitive and conservatively extends existing restrictions. 
Our proof is genuinly algebraic, and h
More precisely, we consider programs  
The
The main finding is tht

==> content/algorithm_unused.tex <==
There are two aspects about $A$ that are inconvenient from an algorithmic point of view.
First, the saturation of $A$ also accepts computations that are reducible.
Second, being a valence system the semantics will restrict the computations to  computations will be checked for being 

There is a run $(\mathit{nop}, \varepsilon)\to (\incdec{o}, w)$ in $\irredof{\ops}$ iff $w.\incdec{o}\in\ops^*$ is irreducible and all prefixes are right-invertible.

Note that the language is the i
%Consider the product valence system $A\times \irredof{\ops}$. 
%As indicated above, n
%Not only Since all runs starting in 
%What is still inconvenient about valence systems is that we 
%We now form the producuct $A\times\irredof{\ops}$ and understand it as a finite automaton with initial state $(q, m$, final state $q'$, and








It remains to ensure such a part is 
which the computation splits.
 which 
 consists of $k^2$
With Proposition~\ref{Proposition:BCSREACHSaturation}, it is sufficient to look for an irreducible computation that multiplies up to one.

Moreover, with 

We give an algorithm that check whether an irreducible computation exists that multiplies up to one, 

To be able to restrict ourselves to irreducible computations, we saturate the valence system such that irreducible computations always exists.

\begin{definition}
\end{definition}



 a computation that 
% ----------------------------------------------------------------
% ----------------------------------------------------------------






















With (summarizing theorem), the task amounts to (i) finding a run over $w$ such that $w\cong w_1\ldots w_n$ decomposes into $n=k^2$ parts $w_1$ to $w_{n}$ such that (ii) each part is irreducible and (iii) the parts freely reduce to $\graphneutral$.  
We address these points and then summarize the algorithm.

Finding a computation that decomposes into $n=k^2$ parts amounts to guessing states $q_1$ to $q_{n-1}$ at which the parts connect and finding computations $w_i$ from $q_{i-1}$ to $q_i$ ($q_{n}=q_f$). 

The second task is to find, given two states $q$ and $q'$ in $A$,  an irreducible computation $u$ from $q$ to $q'$. 
Note that $u$ does not have to be right-invertible.
To get rid of right-invertibility, which is built into the semantics of valence systems, we understand $A$ as a (non-deterministic) automaton $N=(Q, q, \to, \set{q'})$ over the alphabet $\ops$.
It has the same set of states, uses $q$ as the initial state, and has $q'$ as the only final state.  
To obtain irreducible computations, we saturate the NFA.
Intuitively, we enrich the set of transitions by adding $\varepsilon$-transitions for inverses $\inc{o}.\dec{o}$. 
Formally, the \emph{saturation} $\saturation{N}$ is the NFA $(Q, q, \todec, \set{q'})$ where $\to\ \subseteq\ \todec$ is defined by exhaustively applying the following rules:
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
\begin{itemize}
    \item[(i)] If $p_1 \todecw{\inc{o}} p \todecw{}^* p' \todecw{\dec{o}} p_2$, add a transition $p_1 \todecw{\varepsilon} p_2$.
    \item[(ii)] If $p_1 \todecw{\dec{o}} p \todecw{}^* p' \todecw{\inc{o}} p_2$ and $o \indeprel o$, add a transition $p_1 \todecw{\varepsilon} p_2$.    
\end{itemize}
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
\begin{remark}
    In the worst case, we add $\card{Q}^2$-many transitions.
\end{remark}
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
\begin{lemma}
For every $v\in \langof{\saturation{N}}$ there is $u\in\langof{N}$ with $v\cong u$. 
For every $u\in\langof{N}$ there is an irreducible $v\in\langof{\saturation{N}}$ with $u\cong v$.
\end{lemma}
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------

The automaton $\saturation{N}$ still accepts computations that are reducible.
To isolate the irreducible computations, we define another (deterministic) automaton $M$  over the alphabet $\ops$ and form the product with $N$.  
Intuitively, $M$ remembers the last operation and makes sure the next one does not lead to a reduction. 
Formally, $M=(\ops\cup\set{\bot}, \bot, \to, \ops\cup\set{\bot})$ with $\bot\tow{\incdec{o}}\incdec{o}$ and $\incdec{o}\tow{\incdec{a}}\incdec{a}$ for all $o, a\in\ops$ with $a\neq o$.
Moreover, we have $\dec{o}\tow{\inc{o}}\inc{o}$ for all $o\in\ops$ where $o\not\indeprel o$.
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
\begin{lemma}
$\langof{M}=\ops\setminus\Set{w\in\ops^*}{w\text{ is reducible}}$.
\end{lemma}
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
We use $\nfaof{q, q'}$ for the product $N\times M$ whose language is the intersection $\langof{N}\cap \langof{M}$.
This means $\langof{\nfaof{q, q'}}$ consists precisely of the irreducible computations $v$ that lead from $q$ to $q'$.

\begin{comment}
The saturated system $\saturation{A}$ still admits computations that are reducible. 
To isolate the irreducible computations, we define another valence system $M$ and form the product with 
\begin{align*}
B=\saturation{A}\times M\ .
\end{align*}
Intuitively, $M$ checks that two consecutive operations do not lead to a reduction. To this end, it remembers the last operation in its control state.  
Formally, $M=(\ops\cup\set{\bot}, \to)$ with $\bot\tow{\incdec{o}}\incdec{o}$ and $\incdec{o}\tow{\incdec{a}}\incdec{a}$ for all $o\neq a\in\ops$.
Moreover, $\dec{o}\tow{\inc{o}}\inc{o}$ for all $o\in\ops$ where $o\not\indeprel o$.
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
\begin{lemma}\label{Lemma:OnlyIrreducible}
$(\bot, \varepsilon)\to (o, w.o)$ in $M$ iff $w.o\in\ops^*$ is irreducible and right-invertible. 
\end{lemma}
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------

We use $P$ for the set of states in $B$.
The computations will start from $\pinit=(\qinit, \bot)$.
Moreover, we assume to have a state $\pfin$ that is reached from all states $(\qfin, o)$ with an $\varepsilon$-labeled transition. 
With Lemma~\ref{Lemma:Saturate}, $B$ contains the irreducible versions of all computations in $A$.
With Lemma~\ref{Lemma:OnlyIrreducible}, $B$ contains only such computations. 
Since the number of context switches is invariant under saturation, 
we can solve the problem instance on $B$ as follows.
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
\begin{lemma}
\label{Lemma:Saturate}
We have $(\qinit,\varepsilon) \to (\qfin, u)$ with $\cs{u}\leq k$ and $\grapheq{u}=1$ in $A$ iff 
$(\pinit, \varepsilon) \to (\pfin, w)$ with $\cs{w}\leq k$ and $\grapheq{w}=1$ in $B$. Every computation in $B$ is irreducible. 
\end{lemma}
\end{comment}

Whether two computations commute can be checked on the alphabets, $\ops I \ops'$.
Indeed, if we choose the alphabet small enough, it contains precisely the letters from that computation.
More difficult is the question of whether an automaton. 


 freely reduces
}
}
ing the operations in $u$ is ooperation lift the operation of forming syntactic inverses to auto 
With Lemma~, this amounts to checking that $v$ is the syntactic inverse of $u$, $v=\syninv{u}$. 
If $u$ and $v$ are not irreducible, the check may n

Given an automaton $C$ over $\ops$, we define its \emph{}

 All constructions here are polynomial.
 
it is sufficient to guess a test \begin{lemma}\label{Lemma:ReductionAutomataA}
We have $(\qinit,\varepsilon) \to (\qfin,w)$ with $\cs{w}\leq k$ and $\grapheq{w}=1$ in $\saturation{A}$ iff there is a test $\nfa_1$ to $\nfa_n$ and computations $u_1\in\langof{\nfa_1}$ to $u_n\in\langof{\nfa_n}$ that freely reduce to $\graphneutral$.
\end{lemma}

\begin{proof}[Proof Sketch for Theorem~\ref{Theorem:BCSREACHDecidable}]
    \mbox{}\\
    \begin{enumerate}
        \item First saturate the given valence system $A$, obtaining $\saturation{A}$.
        \item Note that it remains to check the existence of an irreducible computation by Proposition~\ref{Proposition:BCSREACHSaturation}.
        \item By Lemma~\ref{Lemma:Crazy}, it is sufficient to check for the existence of a decomposition of length at most $k^2$ that is freely reducible.
        \item For each of the $k$ contexts, guess which symbols are used (and verify that none of them commute).
        \item See Proof of Lemma 30 on Page 19.
    \end{enumerate}
   
\end{proof}


Since the number of context switches is invariant under $\cong$, Lemma~\ref{Lemma:Invariance}, this means we can solve the BCS instance on $\saturation{A}$.

 along one block.It will be a dependent Note that
The function $\tonfa$states are taken from $\saturation{A}$.  
The initial state is $q$, the final state is $q'$. 
The transitions are the ones from $\saturation{A}$, restricted to the given operations $\ops'$.

, we have a sequence of operations on $o$ that either 
next to each other (potentially after) the first rule yields all reductions.
The observation is as follows. 
Given a dependent computation $w$, we can turn it into an irreducible one by applying the following rules  
\begin
To see that this holds, note that dependence rules out  
\rfm{Polish this text.}

Since consider contexts, focus on dependent valence systems.
The key observation is that a sequence of depedent operations is irreducible if and only if there are no consecutive operations
 $\inc{o}.\dec{o}$. can be transformed into an irreduci

For the definition, consider a dependent valence system 
The \emph{saturation} $\saturation{B}$ is


 the blocks there the blocks from the block decompostem
the block decomposition that reduces and the above discussion, there is a computation as required by (BCSREACH) iff there is a test whose automata accept the blocks of the corresponding block decomposition. 


with is , if  and 
there are states $q_0, \ldots, q_{n}$ , dependent sets of operations $\ops_1,\ldots, \ops_k\subseteq \ops$, and subsets $\ops_{j, i}\subseteq \ops_j$ with  so that $$. 

Besides these two operations, we will check whether $\nfa_u$ accepts a computation that reduces to one. 
The reason is that $\nfa_u$ contains all irreducible computations, this amounds to checking whether the automaton accepts $\varepsilon$.
The operation is not needed in the previous section where blocks are assumed to be non-empty.
Here we also track the state changes and have to explicitly discard a block that reduces to one.



==> content/bcs_unused.tex <==
A \emph{context} is a word $w$ such for all $\incdec{o}, \incdec{u}$, $o \neq u$, occurring in $w$, $o$ and $u$ do not commute.
The reader will note that the side condition 

    If $a$ commutes with any letter occurring in $w_k$, then $w_1, \ldots, w_k, a$ is the context-decomposition of $w.a$.
        Else, it is $w_1, \ldots, w_k.a$.
    \end{itemize}

    
    We define $\cs{\varepsilon} = 0$ by convention.
\end{definition}

 the computation 

is that the number of context sw is a subcomputation where where safety verification is undecidable in general. 
The restriction to 
There, the restriction requires that the executing thread  restriction
in the work of   in the sense that the corresponding reachability checks have lo not to consider all computations in order to  that tries to find a violation to 



\rfm{Contexts should not vanish.}


The side condition $w_k\not\cong \graphneutral$ requires contexts (except the last) to have an effect on the memory.
The restriction is for technical convenience, as it allows us to modify the computation using $\cong$ without changing the number of context switches. 
More precisely, we rely on the following lemma.
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
\begin{lemma}\label{Lemma:Invariance}
If $u\cong v$, then $\cs{u}=\cs{v}$.
\end{lemma}
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------
% ---------------------------------------------------------------


%\begin{remark}
%    When analyzing the complexity, we assume that $k$ is encoded in unary.
%\end{remark}


 is the numb $k$.we define its \emph{context decomposition} by induction along the length. 
A single operation is a context. 
Let $w.a$ be a word of length $\geq 2$, and $w_1, \ldots, w_k$ the context decomposition of $w$. 
There are two cases.
\begin{itemize}
\item[(i)] If there is a letter $b\neq a$ in $w_k$ with $a \indeprel b$, then the context decomposition of $w.a$ is $w_1,\ldots, w_k, a$.
\item[(ii)] Otherwise, it is $w_1,\ldots, w_k.a$.
\end{itemize}
The number of \emph{context switches} $\cs{w}$ in a computation $w\in\ops^*$ is the number of contexts in its context decomposition minus one.

 our contribution after having
Our main result is the following

 and based on the saturation a complete check of whether two that admits a block 
We show that full sub
A free reduction is a st either commute orif there is computation, then there is one with a simple shape.
Then we give an algorithm to check whether such a normal-form computation exists.
In a last step, we give a complexity analysis.


\rfm{Indeed, our development applies to a variety of models. Generalizes the basic notion of Rehof and 2006... Moreover, Hague and Lin 2011.}

        \item[\textbf{\frneutralaut}]
            $N_i \frto \varepsilon$, if 
            $\varepsilon\in \langof{N_{i}}$.



==> content/intro_unused.tex <==
%Bounded context switching is an under-approximate verification technique.
%Finding is that it is in NP, for concurrent and recursive programs, potentially communicating via counters. 

%We study the setting of general memories. 
%Valence systems,
%Memories expressed in terms of graph monoids. 

%Contribute a general notion of bounded context switching that applies to programs operating over arbitrary graph monoids.

To this end, the monoid has to be given by some finite description. 
Graph monoids are on the one hand convenient to work with. 
Intuitively 
over graph monoids is i
 in terms of graph monoids, among them concurrent pushdowns but many others. 


Moreover, that reachability under bcs in NP, for all graph monoids.

We assume the memory to be represented by a so-called graph monoid, a standard model in  

a stack among operations that i commutativity among operations.
indicate independence of operations
The edges , and the edges A graph monoid defines the operations via nodes
Graph monoids esta
On the other, they are general enough to capture the


is intuitive and
Intuitive understanding that conservatively generalizes existing results.
On concurrent recursive programs, it will correspond to the classical notion.
On counter systems, it amounts to switching the counter.


and a
The existing tools were limited to , and hence enriches the tool box of g

develop an argument about the shape of computations that uniformly applies to the comp that can handle all memories in a uniform way.


It is algebraic, and understandsWe understand computations as algebraic  single algebraic operations that a computation can be split into qua different from related works that 
rely on a graph interpretation of computations or an encoding into Presburger arithmetic.
give a  
we contribute a new way to think about bounded conte
new approach to thinking about bounded context switching.
The existing algorithms either 
our approach is genuinly algebraic.
An outline of the proof will be given in Section 3, when we have the tools at hand.

is genuin are either graph based or logical
Wheras Madhusudan and Parlato's approach focussed on a graph-theoretic understanding of computations and Hague and Lin emphasized the logical view,  



Logicbase.d




Besides the notion, our study contributes a new proof technique

Claim the following contribution.
\begin{itemize}
	\item General notion of bounded context switching.
\end{itemize}


==> content/prelims_unused.tex <==
   but the operations on the memory.
A memory value $m$ is ch  and the operations aOn the one hand, the 
with a monoid as As our programming model, we consider valence 


\begin{definition}
\end{definition}
%

\begin{remark}
    We can alternatively obtain $\graphmonoid$ as follows:
    Consider $\conginv$, the smallest congruence (with respect to multiplication) on $\tracemonoid{G}$ containing $\traceeq{\inc{o}} \cdot \traceeq{\dec{o}} \conginv \traceneutral$ for all $o$.
    Then we have $\graphmonoid = \tracemonoid / \conginv$.
\end{remark}

 $\incdec{o}.\incdec{u}$ and $\incdec{u}.\incdec{o}$

An edge between two symbols means that the corresponding operations can be used independently. 

We define $\congindep$ as the smallest congruence (with respect to concatenation) on $\ops^*$ containing $\incdec{o} \congindep \incdec{u}$ for all $o \indeprel u$.
We define $\tracemonoid = \ops^* / \congindep$, the \emph{trace monoid} defined by the graph $G$.


\begin{remark}





==> style/abbrev_de.tex <==
% ######################
% ABBREVIATIONS
% ######################

% small
\newcommand{\bzgl}
{bzgl.~}

\newcommand{\obda}
{o.B.d.A.~}

\newcommand{\bzw}
{bzw.~}

\newcommand{\zb}
{z.B.~}

% capital
\newcommand{\Obda}
{O.B.d.A.~}

\newcommand{\Zb}
{Z.B.~}


==> style/abbrev_en.tex <==
% ######################
% ABBREVIATIONS
% ######################

% small
\newcommand{\wrt}
{wrt.~}

\newcommand{\ie}
{i.e.~}

\newcommand{\eg}
{e.g.~}

\newcommand{\resp}
{resp.~}

\newcommand{\sth}
{s.t.~}

\newcommand{\wolog}
{wlog.~}

% capital
\newcommand{\Ie}
{I.e.~}

\newcommand{\Eg}
{E.g.~}

\newcommand{\Wolog}
{Wlog.~}


==> style/algo.tex <==
% ############
% ALGORITHMS
% ############

% algorithms
\usepackage{algorithmicx}
\usepackage{algpseudocode}

%
% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
%

% note that some of the packages above are also needed
\newcommand{\ALGtikzmarkcolor}{black}% customise this, if you want
\newcommand{\ALGtikzmarkextraindent}{4pt}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetstart}{-.5ex}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetend}{-.5ex}% customise this, if you want
\makeatletter
\newcounter{ALG@tikzmark@tempcnta}

\newcommand\ALG@tikzmark@start{%
    \global\let\ALG@tikzmark@last\ALG@tikzmark@starttext%
    \expandafter\edef\csname ALG@tikzmark@\theALG@nested\endcsname{\theALG@tikzmark@tempcnta}%
    \tikzmark{ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname}%
    \addtocounter{ALG@tikzmark@tempcnta}{1}%
}

\def\ALG@tikzmark@starttext{start}
\newcommand\ALG@tikzmark@end{%
    \ifx\ALG@tikzmark@last\ALG@tikzmark@starttext
    % ignore this, the block was opened then closed directly without any other blocks in between (so just a \State basically)
    % don't draw a vertical line here
    \else
    \tikzmark{ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname}%
    \tikz[overlay,remember picture] \draw[\ALGtikzmarkcolor] let \p{S}=($(pic cs:ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetstart)$), \p{E}=($(pic cs:ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetend)$) in (\x{S},\y{S})--(\x{S},\y{E});%
    \fi
    \gdef\ALG@tikzmark@last{end}%
}
% the following line injects our new tikzmarking code
\apptocmd{\ALG@beginblock}{\ALG@tikzmark@start}{}{\errmessage{failed to patch}}
\pretocmd{\ALG@endblock}{\ALG@tikzmark@end}{}{\errmessage{failed to patch}}
\makeatother

%
% end vertical rule patch for algorithmicx
%

\let\Cmd\State

% C-style comments
\renewcommand {\algorithmiccomment}[1]
    {\hfill $/ \!/$ #1}
   
% return on new line
\let\oldReturn\Return
\renewcommand{\Return}{\Cmd\oldReturn}

% commands like in algorith2e
\newcommand {\ForLoop} [2]
{
    \For {#1}
        #2
    \EndFor
}

\newcommand {\WhileLoop} [2]
{
    \While {#1}
        #2
    \EndWhile
}

\newcommand {\IfCond} [2]
{
    \If {#1}
        #2
    \EndIf
}

\newcommand {\IfElseCond} [3]
{
    \If {#1}
        #2
    \Else
        #3
    \EndIf
}


==> style/article.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

%
% Bibliography & references
%

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,maxbibnames=9,maxcitenames=9,backend=bibtex,giveninits=true,isbn=false,doi=false]{biblatex}
\DeclareFieldFormat*{title}{\mkbibitalic{#1\isdot}}
\DeclareFieldFormat*{booktitle}{#1\isdot}
\DeclareFieldFormat*{journaltitle}{#1\isdot}
%\DeclareFieldFormat{titlecase}{\MakeSentenceCase{#1}}
%\newbibmacro*{journal}{%
%    \iffieldundef{journaltitle}
%    {}
%    {\printtext[journaltitle]{%
%            \printfield[noformat]{journaltitle}%
%            \setunit{\subtitlepunct}%
%            \printfield[noformat]{journalsubtitle}}}}

%
% Includes
%

% underlining
\usepackage{ulem}
% set emph back to normal (instead of underlined)
\normalem 

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

%
% TOC and hyperlinks
%
\PassOptionsToPackage{obeyspaces}{url}
\usepackage[bookmarksnumbered]{hyperref} 

% fix nesting in PDF TOC
\usepackage[open=true]{bookmark}


% don't show subsections in TOC
\setcounter{tocdepth}{1}

%
% emph as bold
%

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother
\newcommand{\aemph}[1]{\textit{#1}}


%
% Clever references
%

% clever references
\usepackage{cleveref}
% use capital references by default
\let\scref\cref
\let\cref\Cref


%
% Page layout
%
\usepackage[]{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=2cm, foot=1cm}

\usepackage[headsepline]{scrlayer-scrpage}
%\clearpairofpagestyles
\clearscrheadfoot
\ihead{\normalfont \headmark}
\cfoot{\Large \pagemark}
\automark[]{section}

% space between lines
\onehalfspacing

%
% Hyphenation & separation
%
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%
% Redefined environment
%

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% shortproof without newline
\makeatletter
\newenvironment{shortproof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother


%
% Theorem styles
%

% Theorem numbering
\def\theoremnumberstyle{changesection}

% Theoremstyle
\newtheoremstyle{withnumber} % name
{0.4cm}                      % Space above
{0.6cm}                      % Space below
{\normalfont}                % Body font
{}                           % Indent amount
{\bfseries}                  % Theorem head font
{\newline}                   % Punctuation after theorem head
{0.2cm}                      % Space after theorem head
{#2 #1\thmnote{: \ #3}}      % Theorem head spec (can be left empty, meaning ‘normal’)

\newtheoremstyle{nonumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}              % Body font
{}                         % Indent amount
{\bfseries}                % Theorem head font
{\newline}                 % Punctuation after theorem head
{0.2cm}                    % Space after theorem head
{#1\thmnote{: \ #3}}       % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{withnumber} 

%
% Hackfix for itemize / enumerate at the beginning of a theorem
%
\newcommand{\skipfix}{\leavevmode\vspace{-2.2em}}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \skipfix
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \skipfix
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
%\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
%\usepackage{capt-of}
%\usepackage{caption}
%\DeclareCaptionFont{white}{\color{white}}
%\DeclareCaptionFormat{listing}
%{
%    \colorbox[cmyk]{1, 1, 1,0.01}
%    {
%        \parbox{\textwidth}
%        {\hspace{15pt}#1#2#3}
%    }
%}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
%\usepackage{listings}
%\lstset{
%    numbers=left,
%    numberstyle=\tiny,
%    numbersep=5pt,
%    keywordstyle=\color{black}\bfseries,
%    stringstyle=\ttfamily,
%    showstringspaces=false,
%    basicstyle=\footnotesize,
%    captionpos=b
%}
%\lstset{language=java}
%% Listings
%\lstset{
%    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
%    numbers=left,               % Ort der Zeilennummern
%    numberstyle=\tiny,          % Stil der Zeilennummern
%    %stepnumber=2,               % Abstand zwischen den Zeilennummern
%    numbersep=5pt,              % Abstand der Nummern zum Text
%    tabsize=4,                  % Groesse von Tabs
%    extendedchars=true,         %
%    breaklines=true,            % Zeilen werden Umgebrochen
%    keywordstyle=\text,
%    %frame=b,         
%    stringstyle=\color{black}\ttfamily, % Farbe der String
%    showspaces=false,           % Leerzeichen anzeigen ?
%    showtabs=false,             % Tabs anzeigen ?
%    xleftmargin=5pt,
%    framexleftmargin=17pt,
%    framexrightmargin=5pt,
%    framexbottommargin=4pt,
%    %backgroundcolor=\color{lightgray},
%    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
%    captionpos=t,     
%}
%\lstloadlanguages{% Check Dokumentation for further languages ...
%    %[Visual]Basic
%    %Pascal
%    %C
%    %C++
%    %XML
%    %HTML
%    Java
%}

%
% Colors
%

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}

%
% Boxes for computational problems
%

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
%    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/commands.tex <==
% ##########
% COMMANDS
% ##########

% custom emph
\providecommand {\aemph}[1]
{\textbf{#1}}

% bold + italic
\newcommand {\textbfit} [1]
{\textbf{\textit{#1}}}

% monospace (+ bold & italic)
\newcommand {\mono} [1]
{\texttt{#1}}

\newcommand {\monobf} [1]
{\texttt{\bfseries #1}}

\newcommand {\monobfit} [1]
{\texttt{\bfseries \itshape #1}}

\newcommand {\monoit} [1]
{\texttt{\itshape #1}}

% blackboard bold letters
\providecommand\A{}
\renewcommand {\A} {{\mathbb A}}
\providecommand\B{}
\renewcommand {\B} {{\mathbb B}}
\providecommand{\C}{}
\renewcommand {\C} {{\mathbb C}}
\providecommand\D{}
\renewcommand {\D} {{\mathbb D}}
\providecommand\E{}
\renewcommand {\E} {{\mathbb E}}
\providecommand\F{}
\renewcommand {\F} {{\mathbb F}}
\providecommand {\G} {}
\renewcommand {\G} {{\mathbb G}}
\providecommand\H{}
\renewcommand {\H} {{\mathbb H}}
\providecommand\I{}
\renewcommand {\I} {{\mathbb I}}
\providecommand\J{}
\renewcommand {\J} {{\mathbb J}}
\providecommand\K{}
\renewcommand {\K} {{\mathbb K}}
\providecommand\K{}
\renewcommand {\L} {{\mathbb L}}
\providecommand {\M} {}
\renewcommand {\M} {{\mathbb M}}
\providecommand\N{}
\renewcommand {\N} {{\mathbb N}}
\providecommand\O{}
\renewcommand {\O} {{\mathbb O}}
\providecommand\P{}
\renewcommand {\P} {{\mathbb P}}
\providecommand\Q{}
\renewcommand {\Q} {{\mathbb Q}}
\providecommand\R{}
\renewcommand {\R} {{\mathbb R}}
\providecommand\S{}
\renewcommand {\S} {{\mathbb S}}
\providecommand {\T} {}
\renewcommand {\T} {{\mathbb T}}
\providecommand{\U}{}
\renewcommand {\U} {{\mathbb U}}
\providecommand\V{}
\renewcommand {\V} {{\mathbb V}}
\providecommand\W{}
\renewcommand {\W} {{\mathbb W}}
\providecommand\X{}
\renewcommand {\X} {{\mathbb X}}
\providecommand\Y{}
\renewcommand {\Y} {{\mathbb Y}}
\providecommand\Z{}
\renewcommand {\Z} {{\mathbb Z}}

% calligraphic letters
\newcommand {\calA} {\mathcal{A}}
\newcommand {\calB} {\mathcal{B}}
\newcommand {\calC} {\mathcal{C}}
\newcommand {\calD} {\mathcal{D}}
\newcommand {\calE} {\mathcal{E}}
\newcommand {\calF} {\mathcal{F}}
\newcommand {\calG} {\mathcal{G}}
\newcommand {\calH} {\mathcal{H}}
\newcommand {\calI} {\mathcal{I}}
\newcommand {\calJ} {\mathcal{J}}
\newcommand {\calK} {\mathcal{K}}
\newcommand {\calL} {\mathcal{L}}
\newcommand {\calM} {\mathcal{M}}
\newcommand {\calN} {\mathcal{N}}
\newcommand {\calO} {\mathcal{O}}
\newcommand {\calP} {\mathcal{P}}
\newcommand {\calQ} {\mathcal{Q}}
\newcommand {\calR} {\mathcal{R}}
\newcommand {\calS} {\mathcal{S}}
\newcommand {\calT} {\mathcal{T}}
\newcommand {\calU} {\mathcal{U}}
\newcommand {\calV} {\mathcal{V}}
\newcommand {\calW} {\mathcal{W}}
\newcommand {\calX} {\mathcal{X}}
\newcommand {\calY} {\mathcal{Y}}
\newcommand {\calZ} {\mathcal{Z}}
\newcommand {\cala} {\mathcal{a}}
\newcommand {\calb} {\mathcal{b}}
\newcommand {\calc} {\mathcal{c}}
\newcommand {\cald} {\mathcal{d}}
\newcommand {\cale} {\mathcal{e}}
\newcommand {\calf} {\mathcal{f}}
\newcommand {\calg} {\mathcal{g}}
\newcommand {\calh} {\mathcal{h}}
\newcommand {\cali} {\mathcal{i}}
\newcommand {\calj} {\mathcal{j}}
\newcommand {\calk} {\mathcal{k}}
\newcommand {\call} {\mathcal{l}}
\newcommand {\calm} {\mathcal{m}}
\newcommand {\caln} {\mathcal{n}}
\newcommand {\calo} {\mathcal{o}}
\newcommand {\calp} {\mathcal{p}}
\newcommand {\calq} {\mathcal{q}}
\newcommand {\calr} {\mathcal{r}}
\newcommand {\cals} {\mathcal{s}}
\newcommand {\calt} {\mathcal{t}}
\newcommand {\calu} {\mathcal{u}}
\newcommand {\calv} {\mathcal{v}}
\newcommand {\calw} {\mathcal{w}}
\newcommand {\calx} {\mathcal{x}}
\newcommand {\caly} {\mathcal{y}}
\newcommand {\calz} {\mathcal{z}}

% blackboard bold letters
\newcommand {\bbA} {\mathbb{A}}
\newcommand {\bbB} {\mathbb{B}}
\newcommand {\bbC} {\mathbb{C}}
\newcommand {\bbD} {\mathbb{D}}
\newcommand {\bbE} {\mathbb{E}}
\newcommand {\bbF} {\mathbb{F}}
\newcommand {\bbG} {\mathbb{G}}
\newcommand {\bbH} {\mathbb{H}}
\newcommand {\bbI} {\mathbb{I}}
\newcommand {\bbJ} {\mathbb{J}}
\newcommand {\bbK} {\mathbb{K}}
\newcommand {\bbL} {\mathbb{L}}
\newcommand {\bbM} {\mathbb{M}}
\newcommand {\bbN} {\mathbb{N}}
\newcommand {\bbO} {\mathbb{O}}
\newcommand {\bbP} {\mathbb{P}}
\newcommand {\bbQ} {\mathbb{Q}}
\newcommand {\bbR} {\mathbb{R}}
\newcommand {\bbS} {\mathbb{S}}
\newcommand {\bbT} {\mathbb{T}}
\newcommand {\bbU} {\mathbb{U}}
\newcommand {\bbV} {\mathbb{V}}
\newcommand {\bbW} {\mathbb{W}}
\newcommand {\bbX} {\mathbb{X}}
\newcommand {\bbY} {\mathbb{Y}}
\newcommand {\bbZ} {\mathbb{Z}}
\newcommand {\bba} {\mathbb{a}}
\newcommand {\bbb} {\mathbb{b}}
\newcommand {\bbc} {\mathbb{c}}
\newcommand {\bbd} {\mathbb{d}}
\newcommand {\bbe} {\mathbb{e}}
\newcommand {\bbf} {\mathbb{f}}
\newcommand {\bbg} {\mathbb{g}}
\newcommand {\bbh} {\mathbb{h}}
\newcommand {\bbi} {\mathbb{i}}
\newcommand {\bbj} {\mathbb{j}}
\newcommand {\bbk} {\mathbb{k}}
\newcommand {\bbl} {\mathbb{l}}
\newcommand {\bbm} {\mathbb{m}}
\newcommand {\bbn} {\mathbb{n}}
\newcommand {\bbo} {\mathbb{o}}
\newcommand {\bbp} {\mathbb{p}}
\newcommand {\bbq} {\mathbb{q}}
\newcommand {\bbr} {\mathbb{r}}
\newcommand {\bbs} {\mathbb{s}}
\newcommand {\bbt} {\mathbb{t}}
\newcommand {\bbu} {\mathbb{u}}
\newcommand {\bbv} {\mathbb{v}}
\newcommand {\bbw} {\mathbb{w}}
\newcommand {\bbx} {\mathbb{x}}
\newcommand {\bby} {\mathbb{y}}
\newcommand {\bbz} {\mathbb{z}}

% letters in Fraktur
\newcommand {\frakA} {\mathfrak{A}}
\newcommand {\frakB} {\mathfrak{B}}
\newcommand {\frakC} {\mathfrak{C}}
\newcommand {\frakD} {\mathfrak{D}}
\newcommand {\frakE} {\mathfrak{E}}
\newcommand {\frakF} {\mathfrak{F}}
\newcommand {\frakG} {\mathfrak{G}}
\newcommand {\frakH} {\mathfrak{H}}
\newcommand {\frakI} {\mathfrak{I}}
\newcommand {\frakJ} {\mathfrak{J}}
\newcommand {\frakK} {\mathfrak{K}}
\newcommand {\frakL} {\mathfrak{L}}
\newcommand {\frakM} {\mathfrak{M}}
\newcommand {\frakN} {\mathfrak{N}}
\newcommand {\frakO} {\mathfrak{O}}
\newcommand {\frakP} {\mathfrak{P}}
\newcommand {\frakQ} {\mathfrak{Q}}
\newcommand {\frakR} {\mathfrak{R}}
\newcommand {\frakS} {\mathfrak{S}}
\newcommand {\frakT} {\mathfrak{T}}
\newcommand {\frakU} {\mathfrak{U}}
\newcommand {\frakV} {\mathfrak{V}}
\newcommand {\frakW} {\mathfrak{W}}
\newcommand {\frakX} {\mathfrak{X}}
\newcommand {\frakY} {\mathfrak{Y}}
\newcommand {\frakZ} {\mathfrak{Z}}
\newcommand {\fraka} {\mathfrak{a}}
\newcommand {\frakb} {\mathfrak{b}}
\newcommand {\frakc} {\mathfrak{c}}
\newcommand {\frakd} {\mathfrak{d}}
\newcommand {\frake} {\mathfrak{e}}
\newcommand {\frakf} {\mathfrak{f}}
\newcommand {\frakg} {\mathfrak{g}}
\newcommand {\frakh} {\mathfrak{h}}
\newcommand {\fraki} {\mathfrak{i}}
\newcommand {\frakj} {\mathfrak{j}}
\newcommand {\frakk} {\mathfrak{k}}
\newcommand {\frakl} {\mathfrak{l}}
\newcommand {\frakm} {\mathfrak{m}}
\newcommand {\frakn} {\mathfrak{n}}
\newcommand {\frako} {\mathfrak{o}}
\newcommand {\frakp} {\mathfrak{p}}
\newcommand {\frakq} {\mathfrak{q}}
\newcommand {\frakr} {\mathfrak{r}}
\newcommand {\fraks} {\mathfrak{s}}
\newcommand {\frakt} {\mathfrak{t}}
\newcommand {\fraku} {\mathfrak{u}}
\newcommand {\frakv} {\mathfrak{v}}
\newcommand {\frakw} {\mathfrak{w}}
\newcommand {\frakx} {\mathfrak{x}}
\newcommand {\fraky} {\mathfrak{y}}
\newcommand {\frakz} {\mathfrak{z}}

% script letters
\newcommand {\scrA} {\mathscr{A}}
\newcommand {\scrB} {\mathscr{B}}
\newcommand {\scrC} {\mathscr{C}}
\newcommand {\scrD} {\mathscr{D}}
\newcommand {\scrE} {\mathscr{E}}
\newcommand {\scrF} {\mathscr{F}}
\newcommand {\scrG} {\mathscr{G}}
\newcommand {\scrH} {\mathscr{H}}
\newcommand {\scrI} {\mathscr{I}}
\newcommand {\scrJ} {\mathscr{J}}
\newcommand {\scrK} {\mathscr{K}}
\newcommand {\scrL} {\mathscr{L}}
\newcommand {\scrM} {\mathscr{M}}
\newcommand {\scrN} {\mathscr{N}}
\newcommand {\scrO} {\mathscr{O}}
\newcommand {\scrP} {\mathscr{P}}
\newcommand {\scrQ} {\mathscr{Q}}
\newcommand {\scrR} {\mathscr{R}}
\newcommand {\scrS} {\mathscr{S}}
\newcommand {\scrT} {\mathscr{T}}
\newcommand {\scrU} {\mathscr{U}}
\newcommand {\scrV} {\mathscr{V}}
\newcommand {\scrW} {\mathscr{W}}
\newcommand {\scrX} {\mathscr{X}}
\newcommand {\scrY} {\mathscr{Y}}
\newcommand {\scrZ} {\mathscr{Z}}
\newcommand {\scra} {\mathscr{a}}
\newcommand {\scrb} {\mathscr{b}}
\newcommand {\scrc} {\mathscr{c}}
\newcommand {\scrd} {\mathscr{d}}
\newcommand {\scre} {\mathscr{e}}
\newcommand {\scrf} {\mathscr{f}}
\newcommand {\scrg} {\mathscr{g}}
\newcommand {\scrh} {\mathscr{h}}
\newcommand {\scri} {\mathscr{i}}
\newcommand {\scrj} {\mathscr{j}}
\newcommand {\scrk} {\mathscr{k}}
\newcommand {\scrl} {\mathscr{l}}
\newcommand {\scrm} {\mathscr{m}}
\newcommand {\scrn} {\mathscr{n}}
\newcommand {\scro} {\mathscr{o}}
\newcommand {\scrp} {\mathscr{p}}
\newcommand {\scrq} {\mathscr{q}}
\newcommand {\scrr} {\mathscr{r}}
\newcommand {\scrs} {\mathscr{s}}
\newcommand {\scrt} {\mathscr{t}}
\newcommand {\scru} {\mathscr{u}}
\newcommand {\scrv} {\mathscr{v}}
\newcommand {\scrw} {\mathscr{w}}
\newcommand {\scrx} {\mathscr{x}}
\newcommand {\scry} {\mathscr{y}}
\newcommand {\scrz} {\mathscr{z}}

% fake capital Greek letters for the sake of complenetess
% upright (instead of italic/slanted) to match the other Greek capitals
%\providecommand{\Alpha} {}
%\renewcommand {\Alpha} {\mathsf{A}}
%\providecommand{\Beta} {}
%\renewcommand {\Beta} {\mathsf{B}}
%\providecommand{\Epsilon} {}
%\renewcommand {\Epsilon} {\mathsf{E}}
%\providecommand{\Zeta} {}
%\renewcommand {\Zeta} {\mathsf{Z}}
%\providecommand{\Eta} {}
%\renewcommand {\Eta} {\mathsf{H}}
%\providecommand{\Iota} {}
%\renewcommand {\Iota} {\mathsf{I}}
%\providecommand{\Kappa} {}
%\renewcommand {\Kappa} {\mathsf{K}}
%\providecommand{\Mu} {}
%\renewcommand {\Mu} {\mathsf{M}}
%\providecommand{\Tau} {}
%\renewcommand {\Tau} {\mathsf{T}}
%\providecommand{\Chi} {}
%\renewcommand {\Chi} {\mathsf{X}}


==> style/definitions.tex <==
% ##################
% DEFINITIONS
% ##################

%
% Basic stuff
%

\newcommand { \from }
{ \leftarrow }

\newcommand {\Rplus} 
{ \R_{>0} }

\newcommand {\true}
{\mathit{true}}

\newcommand {\false}
{\mathit{false}}

\newcommand {\monotrue}
{\mathtt{true}}

\newcommand {\monofalse}
{\mathtt{false}}

\newcommand {\ifalse}
{\mathit{false}}

\newcommand {\itrue}
{\mathit{true}}

\newcommand {\oneto} [1]
{\left\{ 1, \ldots, #1\right\}}

\newcommand {\zeroto} [1]
{\left\{ 0, \ldots, #1\right\}}

\newcommand {\arity} [1]
{ {\scriptstyle / #1 } }

% small @
\newcommand {\at}
{
    \raisebox{0.5mm}{\scalebox{0.7}[0.7]{@}}
}

% corresponds to
\newcommand\corrto{%
    \let\savearraystretch\arraystretch
    \renewcommand\arraystretch{0.3}
    \begin{array}{c}
        \stretchto{
            \scalerel*[\widthof{=}]{\wedge}
            {\rule{1ex}{3ex}}%
        }{0.5ex}\\ 
        =%
    \end{array}
    \let\arraystretch\savearraystretch
}

% stacked logical operators
\newcommand{\wedgevee}
{
    \mathrel{\substack{\wedge\\\vee}}
}
\newcommand{\veewedge}
{
    \mathrel{\substack{\vee\\\wedge}}
}

% small mid for (E)BNF
\newcommand{\bnf}
{\:\shortmid\:}

%
% Sets
%

\newcommand{\card}[1]
{\left|#1\right|}

\newcommand {\set} [1]
{ \left\{ #1 \right\} }

\newcommand {\Set} [2]
{ \left\{ #1 \ \middle| \ #2 \right\} }

\newcommand {\smallset} [2]
{ \{ #1 \mid #2 \} }

\newcommand {\ideal} [1]
{ \langle \ #1 \ \rangle}

\newcommand {\Ideal} [2]
{ \langle \ #1 \mid #2 \ \rangle}

\newcommand {\pwrset} [1]
{ {\mathcal P} \left( #1 \right)}

%
% Set operations
%

% disjoint union
\makeatletter
\providecommand*{\bigdotcup}{%
    \mathbin{%
        \mathpalette\@bigdotcup{}%
    }%
}
\newcommand*{\@bigdotcup}[2]{%
    \ooalign{%
        $\m@th#1\bigcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\providecommand*{\dotcup}{%
    \mathbin{%
        \mathpalette\@dotcup{}%
    }%
}
\newcommand*{\@dotcup}[2]{%
    \ooalign{%
        $\m@th#1\cup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\providecommand*{\bigdotsqcup}{%
    \mathbin{%
        \mathpalette\@bigdotsqcup{}%
    }%
}
\newcommand*{\@bigdotsqcup}[2]{%
    \ooalign{%
        $\m@th#1\bigsqcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\providecommand*{\dotsqcup}{%
    \mathbin{%
        \mathpalette\@dotsqcup{}%
    }%
}
\newcommand*{\@dotsqcup}[2]{%
    \ooalign{%
        $\m@th#1\sqcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

%
% Closures
%

\newcommand{\up}
{\!\uparrow}

\newcommand{\down}
{\!\downarrow}

\newcommand{\dc}[1]
{#1\down }

\newcommand{\uc}[1]
{#1\up }

%
% Logic
%

% semantic brackets
\newcommand {\sem}[1]
{	\left\llbracket #1 \right\rrbracket }

% inverse models
\makeatletter
\providecommand*{\Dashv}{%
    \mathrel{%
        \mathpalette\@Dashv\vDash
    }%
}
\makeatother

% logical equivalence (\models \ismod)
\newcommand{\lequiv}{\vDash\hspace{-2pt}\Dashv}

%
% Complexity
%

\newcommand {\bigO} [1]
{ \calO \left( {#1} \right) }

\newcommand {\smallO} [1]
{ o \left( #1 \right) }

\newcommand {\bigOmega} [1]
{ \Omega \left( #1 \right) }

\newcommand {\smallOmega} [1]
{ \omega \left( #1 \right) }

\newcommand {\bigTheta} [1]
{ \Theta \left( #1 \right) }

% blank symbol
\newsavebox{\blankbox}
\savebox{\blankbox}{\texttt{aa}}
\newcommand\vartextvisiblespace[1][0.8\wd\blankbox]{%
    \makebox[#1]{\kern.1em\rule{.4pt}{.5ex}%
        \hrulefill%
        \rule{.4pt}{.5ex}\kern.1em}%
}
\newcommand{\blank}{\vartextvisiblespace}% For ease-of-use


\newcommand {\LOGSPACE}
{\mathsf{L}}
\newcommand {\NLOGSPACE}
{\mathsf{NL}}
\newcommand {\PTIME}
{\mathsf{P}}
\newcommand {\NPTIME}
{\mathsf{NP}}
\newcommand {\PSPACE}
{\mathsf{PSPACE}}
\newcommand {\EXPTIME}
{\mathsf{EXP}}
\newcommand {\EXPSPACE}
{\mathsf{EXPSPACE}}

%
% Words
%

\newcommand {\subword}
{\!\preceq}

%
% Automata theory
%

\newcommand {\tow} [1]
{ \xrightarrow{#1} }

\newcommand{\towin}[2]
{\tow{#1}_{#2}}

\DeclareDocumentCommand \lang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL }
    { \calL \left( #1 \right) }
}

\DeclareDocumentCommand \olang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL^\omega }
    { \calL^\omega \!\left( #1 \right) }
}

\DeclareDocumentCommand \Parikh { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \Psi }
    { \Psi \left( #1 \right) }
}

%
% Grammars
%

% derivation
\newcommand{\derive}{\Rightarrow}
\newcommand{\leftderive}{\derive}

%
% Special
%

\newcommand{\Buechi}{B\"uchi}


==> style/eptcs_additions.tex <==
% #####################
% ADDITIONS FOR LIPICS
% #####################
% some paper specific stuff

% enumerate[a)] etc.
\usepackage{paralist}

\usepackage{amssymb}

\usepackage{amsthm}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem {proposition} [theorem] {Proposition}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}

% separation rules
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

% Quotes
\newcommand {\quot} [1] {\enquote{#1}}


% Boxes for computation problems
%
%
\newcommand{\ProblemLocGiven}{Given}
\newcommand{\ProblemLocDecide}{Decide}
\newcommand{\ProblemLocCompute}{Compute}

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question


\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \sffamily
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \sffamily
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/exam.tex <==
% ########################
% EXAM SPECIFIC STUFF
% ########################

% underlining
\usepackage{ulem}
% set emph back to normal (instead of underlined)
\normalem 

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

%
% TOC and hyperlinks
%
\PassOptionsToPackage{obeyspaces}{url}
\usepackage[bookmarksnumbered]{hyperref} 

% border size
\usepackage{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2cm, bottom=2cm, foot= 1cm}

\usepackage[headsepline]{scrlayer-scrpage}
%\clearpairofpagestyles
\clearscrheadfoot
%\ihead{\normalfont \headmark}
\ohead{\hfill \quad \normalfont \page{} \pagemark~/~\Nrpages}
%\automark[]{section}

%
% Dot after section number
%
\usepackage{secdot}
\sectionpunct{subsection}{ }

% space between lines
\onehalfspacing

%
% Hyphenation & separation
%
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%
% Clever references
%

% clever references
\usepackage{cleveref}
% use capital references by default
\let\scref\cref
\let\cref\Cref
% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother
\newcommand{\aemph}[1]{\textit{#1}}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
%\lstset{language=java}
%% Listings
%\lstset{
%    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
%    numbers=left,               % Ort der Zeilennummern
%    numberstyle=\tiny,          % Stil der Zeilennummern
%    %stepnumber=2,               % Abstand zwischen den Zeilennummern
%    numbersep=5pt,              % Abstand der Nummern zum Text
%    tabsize=4,                  % Groesse von Tabs
%    extendedchars=true,         %
%    breaklines=true,            % Zeilen werden Umgebrochen
%    keywordstyle=\text,
%    %frame=b,         
%    stringstyle=\color{black}\ttfamily, % Farbe der String
%    showspaces=false,           % Leerzeichen anzeigen ?
%    showtabs=false,             % Tabs anzeigen ?
%    xleftmargin=5pt,
%    framexleftmargin=17pt,
%    framexrightmargin=5pt,
%    framexbottommargin=4pt,
%    %backgroundcolor=\color{lightgray},
%    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
%    captionpos=t,     
%}
%
%\lstloadlanguages{% Check Dokumentation for further languages ...
%    %[Visual]Basic
%    %Pascal
%    %C
%    %C++
%    %XML
%    %HTML
%    Java
%}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}


%
% Boxes for computational problems
%

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother

\newenvironment{firstpage}
{
    \thispagestyle{empty}
    \newgeometry{top=1cm, bottom=1cm}
}
{
    \pagebreak
    \restoregeometry
}



%
% Exam special stuff
%

\newcommand{\statement}[1]{
    #1	& $\Box$ & $\Box$ \\
}

\newcommand{\maxpts}[1]
{
    \vspace*{-1.5cm}
    \hfill \fbox{\large #1 \pts}
    \vspace*{1cm}
}



% multiplechoice
\newenvironment{multiplechoice}[2]{
    \begin{center}
        \begin{tabular}{lcc}
            & #1 & #2 \\
        }{
        \end{tabular}
    \end{center}
    \vspace{0.5cm}
}

\newenvironment{exerciseDE}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
    
}
{
}

\newenvironment{exerciseEN}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
    
}
{
}

\usepackage{verbatim}

\makeatletter
\def\destring{de}
\ifx\style@lang\destring % German

% for comment / endcomment

\newcommand{\exinclude}[1]
{
    \input{exercises/#1}
}

\renewenvironment{exerciseEN}[2]
{
    \comment
}
{
    \endcomment
}


\else % English

\newcommand{\exinclude}[1]
{
    \input{exercises/#1}
}

\renewenvironment{exerciseDE}[2]
{
    \comment
}
{
    \endcomment
}

\fi
\makeatother



==> style/exsheet.tex <==
% ##############################
% EXERCISE SHEET SPECIFIC STUFF
% ##############################

%
% Bibliography & references
%

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,maxbibnames=9,maxcitenames=9,backend=bibtex,giveninits=true,isbn=false,doi=false]{biblatex}
\DeclareFieldFormat*{title}{\mkbibitalic{#1\isdot}}
\DeclareFieldFormat*{booktitle}{#1\isdot}
\DeclareFieldFormat*{journaltitle}{#1\isdot}
%\DeclareFieldFormat{titlecase}{\MakeSentenceCase{#1}}
%\newbibmacro*{journal}{%
%    \iffieldundef{journaltitle}
%    {}
%    {\printtext[journaltitle]{%
%            \printfield[noformat]{journaltitle}%
%            \setunit{\subtitlepunct}%
%            \printfield[noformat]{journalsubtitle}}}}

%
% Includes
%

% underlining
\usepackage{ulem}
% set emph back to normal (instead of underlined)
\normalem 

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% border size
\usepackage[]{geometry}
\geometry{left=2.2cm, right=2.2cm, top=2cm, bottom=2cm, foot= 1cm}

%
% emph as bold
%

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother
\newcommand{\aemph}[1]{\textit{#1}}

%
% Clever references
%

% clever references
\usepackage{cleveref}
% use capital references by default
\let\scref\cref
\let\cref\Cref

\usepackage{scrlayer-scrpage}
\clearscrheadfoot

% space between lines
\onehalfspacing

%
% Hyphenation & separation
%
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%
% Redefined environment
%

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
    {paragraph} % name
    {4}         % level
    {\z@}       % indent     
    {0ex \@plus -1ex \@minus -.2ex} % beforeskip
    %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
    {0.01ex \@plus .2ex}                % afterskip
    %{1.5ex \@plus -2ex}                % afterskip
    {\normalfont\normalsize\bfseries} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% shortproof without newline
\makeatletter
\newenvironment{shortproof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother


%
% Theorem styles
%

% Theoremstyle
\newtheoremstyle{withnumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1 #2\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\newtheoremstyle{nonumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{withnumber} 

%
% Hackfix for itemize / enumerate at the beginning of a theorem
%
\newcommand{\skipfix}{\leavevmode\vspace{-2.2em}}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \skipfix
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \skipfix
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
%\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
%\usepackage{capt-of}
%\usepackage{caption}
%\DeclareCaptionFont{white}{\color{white}}
%\DeclareCaptionFormat{listing}
%{
%    \colorbox[cmyk]{1, 1, 1,0.01}
%    {
%        \parbox{\textwidth}
%        {\hspace{15pt}#1#2#3}
%    }
%}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
%\usepackage{listings}
%\lstset{
%    numbers=left,
%    numberstyle=\tiny,
%    numbersep=5pt,
%    keywordstyle=\color{black}\bfseries,
%    stringstyle=\ttfamily,
%    showstringspaces=false,
%    basicstyle=\footnotesize,
%    captionpos=b
%}
%\lstset{language=java}
%% Listings
%\lstset{
%    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
%    numbers=left,               % Ort der Zeilennummern
%    numberstyle=\tiny,          % Stil der Zeilennummern
%    %stepnumber=2,               % Abstand zwischen den Zeilennummern
%    numbersep=5pt,              % Abstand der Nummern zum Text
%    tabsize=4,                  % Groesse von Tabs
%    extendedchars=true,         %
%    breaklines=true,            % Zeilen werden Umgebrochen
%    keywordstyle=\text,
%    %frame=b,         
%    stringstyle=\color{black}\ttfamily, % Farbe der String
%    showspaces=false,           % Leerzeichen anzeigen ?
%    showtabs=false,             % Tabs anzeigen ?
%    xleftmargin=5pt,
%    framexleftmargin=17pt,
%    framexrightmargin=5pt,
%    framexbottommargin=4pt,
%    %backgroundcolor=\color{lightgray},
%    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
%    captionpos=t,     
%}
%\lstloadlanguages{% Check Dokumentation for further languages ...
%    %[Visual]Basic
%    %Pascal
%    %C
%    %C++
%    %XML
%    %HTML
%    Java
%}

%
% Colors
%

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}

%
% Boxes for computational problems
%

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}

\makeatother
\newtoks\lecturer
\newtoks\organizer
\newtoks\institution
\newtoks\term
\newtoks\releasedate
\newtoks\duedate

\makeatletter
\newcommand{\head}
{
    %   \newgeometry{top=1cm}
    \vspace*{-3\baselineskip}
    %\null
    %\thispagestyle{empty}
    %\begin{center} 
    \framebox[\textwidth]{
        \parbox{\textwidth}
        {
            \vspace*{-0.2cm}
            \begin{center}
                \textrm{\textbf{\large \@title}} \\
                \textrm{\textbf{\large \@subtitle}}
            \end{center}
            \vspace*{-0.9cm}
            \begin{tabu} to \textwidth {l X r}
                \small \the\lecturer  & & \small \the\institution \\
                \small \the\organizer  & & \small \the\term \\
            \end{tabu}
        }
    } 
    %\end{center}
    %\null
    \begin{tabu} to \textwidth {@{} l X r @{}}
        \the\releasedate  & & \the \duedate \\
    \end{tabu}
    %    \vspace*{0.2cm}
    %    \restoregeometry
}
\makeatother


==> style/ieee_additions.tex <==
% #####################
% ADDITIONS FOR IEEE
% #####################

% enumerate[a)] etc
\usepackage{paralist}

% define theorem styles
\theoremstyle{plain}

\newtheorem {theorem}       {Theorem}     []
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Exercise}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

% separation rules
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%compact llncs-like paragraph
\newcommand{\compactparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}

\newcommand{\subparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}


==> style/includes.tex <==
% ##########
% INCLUDES
% ##########

% images, ...
\usepackage{graphicx}

% tables (over several pages)
\usepackage{tabu}

% boxes in the text
\usepackage{fancybox}

% math symbols
\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{stmaryrd} 
\usepackage{amsthm}
\usepackage{wasysym}
\usepackage{marvosym}

% for coloring stuff
\usepackage{xcolor}

% for colored cells in tables
\usepackage{colortbl}

% symbol scaling in math mode
\usepackage{scalerel}

% for symbol stacking
\usepackage{stackengine}

% parse optional arguments
\usepackage{xparse}

% fix some spacing issues
\usepackage{microtype}

% custom environments
\usepackage{environ}


==> style/lang_de.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: DEUTSCH
% ###################################

%
% Packages
%

%\usepackage{polyglossia}
%\setdefaultlanguage{german}

%\usepackage[ngerman]{babel}

\usepackage[utf8]{inputenc}
\usepackage{csquotes}

%
% Quotes
%

\newcommand {\quot} [1] {\enquote{#1}}

%
% Commands
%

\newcommand{\pts}{Punkte}
\newcommand{\page}{Seite}
\newcommand{\ProblemLocGiven}{Gegeben}
\newcommand{\ProblemLocDecide}{Entscheide}
\newcommand{\ProblemLocCompute}{Berechne}




==> style/lang_en.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: ENGLISH
% ###################################

%
% Packages
%

\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{csquotes}


%
% Quotes
% 

\newcommand {\quot} [1] {\enquote{#1}}

%
% Commands
%

\newcommand{\pts}{points}
\newcommand{\page}{Page}
\newcommand{\ProblemLocGiven}{Given}
\newcommand{\ProblemLocDecide}{Decide}
\newcommand{\ProblemLocCompute}{Compute}



==> style/letter.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% remove all paragraph indentation
\usepackage{parskip}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

% abbreviation index
\usepackage[german]{nomencl}
\let\abbrev\nomenclature

% border size
\usepackage{geometry}
% top is later changed, just for title page
\geometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

%\usepackage{scrpage2}
%\pagestyle{scrheadings}
%\cfoot{\pagemark}

%  headline / footline
\usepackage{fancyhdr} %Paket laden
\pagestyle{fancy} %eigener Seitenstil

%% Seitennummer immer oben rechts
%% alle Kopf- und Fußzeilenfelder bereinigen
%\fancyhf{}
%% Kopfzeile links: Name des Kapitels = der Sektion
%\fancyhead[L]{\nouppercase{\leftmark}}
%% Kopfzeile zentriert:
%\fancyhead[C]{} 
%% Kopfzeile rechts = Seitennummer
%\fancyhead[R]{\thepage} 
%% Trennlinien
%\renewcommand{\headrulewidth}{0.4pt} 
%%\renewcommand{\footrulewidth}{0.4pt}
%% Analog
%%\fancyfoot[C]{\thepage}


% Seitennummer immer oben rechts
% alle Kopf- und Fußzeilenfelder bereinigen
\fancyhf{}
\fancyfoot[C]{\thepage}
\renewcommand{\headrule}{} 

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Zu verwendende Regelsaetze 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
%%% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
%%% zusaetzlichen Punkt.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\swappedhead#1#2#3{%
%    \thmnumber{#2}\thmname{\@ifnotempty{#2}{ }#1}%
%    \thmnote{ {\the\thm@notefont(#3)}}}

\def\swappedhead#1#2#3{%
    \thmnumber{#2}\thmname{ #1}%
    \thmnote{ {\the\thm@notefont(#3)}}}

\newtheoremstyle{varthm-roman-break}% name
{}%      Space above, empty = `usual value'
{}%      Space below
{\normalfont}% Body font
{}%         Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{}%        Punctuation after thm head
{\newline}%     Space after thm head: " " = normal interword space;
%       \newline = linebreak
{\thmnote{#3}}% Thm head spec


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Eigene Befehle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Label an beliebiger Stelle mit beliebigem Symbol setzen
% \mylabel{labelname}{(*)} liefert (*) nach \ref{labelname}
\catcode`@=11%%% Sorgt daruer, dass @ in Marconamen verwendet werden kann
\newcommand{\mylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}}}%
    \@esphack}
\newcommand{\tmylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}{\arabic{chapter}}}}%
    \@esphack}
\catcode`@=\active%
%%% Erzeugt an der Stelle des Aufrufs einen nicht sichtbaren Punkt.
\newcommand{\leererpunkt}{
    \drawdim pt
    \begin{texdraw}
        \setgray 1
        \lcir r:0.01       
    \end{texdraw}
}

\swapnumbers
\theoremstyle{varthm-roman-break} 

\newtheorem {theorem}	    {Theorem}     [section]
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Example}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }


% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
\captionsetup[lstlisting]
{
    format=listing,
    labelfont=white,
    textfont=white,
    singlelinecheck=false,
    margin=0pt,
    font={bf,footnotesize}
}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}


\newtoks\receiver
\newtoks\address
\newtoks\postalbox
\newtoks\plz
\newtoks\telnr
\newtoks\email

\catcode`\@ = 11 % Macro \makeatletter does the same

%\newcommand{ \at } { \makeatletter @ \makeatother }

\newcommand {\letterhead}
{
    
    \begin{tabu} to \textwidth {lXr}
        \large \the\receiver       & & \large Sebastian Muskalla\\
        \small \the\address     & & \small Institut für Theoretische Informatik\\
        \small \the\postalbox  & & \small Mühlenpfordtstr. 23\\
        \small \the\plz       & & \small 38106 Braunschweig\\
        \small \the\telnr     & & \small Tel.:  +49 (0)531 391 9520 \\
        \small \the\email     & & \small E-Mail: s.muskalla{\!\at \!}tu-bs.de\\
                                & & \\
                                & & Braunschweig, den \today \\
    \end{tabu}
    \makeatother
}

\newcommand {\lettertitle}
{\mbox{}\\\textbf{\Large{\@title}}\\}




==> style/lipics_additions.tex <==
% #####################
% ADDITIONS FOR LIPICS
% #####################
% some paper specific stuff

% enumerate[a)] etc.
\usepackage{paralist}

\theoremstyle{plain}
\newtheorem {proposition} [theorem] {Proposition}
\newtheorem {claim} [theorem] {Claim}

\theoremstyle{definition}
\newtheorem {algo} [theorem] {Algorithm}
\newtheorem {rmk} [theorem] {Remark}

% separation rules
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

% Quotes
\newcommand {\quot} [1] {\enquote{#1}}


% Boxes for computation problems
%
%
\newcommand{\ProblemLocGiven}{Given}
\newcommand{\ProblemLocDecide}{Decide}
\newcommand{\ProblemLocCompute}{Compute}

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question


\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \sffamily
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{0.5\parindent}} l X c}
            \multicolumn{2}{@{\hspace{0.5\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \sffamily
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{0.5\parindent}} l X c}
            \multicolumn{2}{@{\hspace{0.5\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/misc.tex <==
% ##########
% MISC
% ##########

%
% Fix delimiter spacing
%
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

%
% Custom symbols
%

% triangle qed
\newcommand{\tqed}{\hfill \text{$\blacktriangleleft$}}

% item with arrow symbol like in Meyer's lectures
\newcommand {\itemarrow} 
{ {\raisebox{0.8mm}{\rotatebox[origin=c]{180}{$\Lsh$}}} } 

%
% Use slanted versions of leq & geq by default
%

% store old symbols
\let\leqstraight\leq % or just use le
\let\geqstraight\geq % or just use ge
\let\nleqstraight\nleq
\let\ngeqstraight\ngeq
\let\nle\nleq
\let\nge\ngeq

% overwrite
\let\leq\leqslant
\let\geq\geqslant
\let\nleq\leqslant
\let\ngeq\ngeqslant


==> style/myriad.tex <==
% #######
% MYRIAD
% #######

%
% Use Myriad Pro for text and math
%

% MdSymbol for math symbols that work well together with Myriad Pro
\usepackage{mdsymbol}

% Mathspec to change fonts for math and text
% (loads fontspecc with no-math option)
\usepackage{mathspec}

% Use Myriad Pro for text
\setmainfont{Myriad Pro}
\setsansfont{Myriad Pro}

% Use Myriad Pro for math
\setmathsfont(Digits,Latin,Greek){Myriad Pro}
\setmathrm{Myriad Pro}
\setmathsf{Myriad Pro}

% Use Consolas as monospace / typewriter font for text an math
\setmonofont{Consolas}
\setmathtt{Consolas}

% the greek symbols provided by Myriad Pro already look like their standard-LaTeX var-variants
\let\oldvarepsilon\varepsilon
\let\oldvarphi\varphi
\let\varepsilon\epsilon
\let\varphi\phi

% Load font styles for math that are not included in Myriad Pro
% Blackboard bold: Boondox (which is based on STIX)
% Calligraphic: Computer Modern (simply the best...)
% Fraktur: Boondox (which is based on STIX)
% Boondox (based on stix) for, fraktur and script
% Script: Boondox
\usepackage
[
    cal=cm,
    bb=boondox,
    frak=boondox,
    scr=boondoxo
]
{mathalfa}

\let\oldell\ell
\renewcommand{\ell}{\mathscr{l}}

% bm for bold math
% does not work with greek letters - but Myriad Pro provides bold greek letters, available using \mathbf
\usepackage{bm}

% hack for correct bold Greek letters

\newcommand{\bAlpha}{\bm{Alpha}}

%$\Alpha \Beta \Gamma \Delta \Epsilon \Zeta \Eta \Theta \Iota \Kappa \Lambda \Mu \Nu \Xi O \Pi \Rho \Sigma \Tau \Upsilon \Phi \Chi \Psi \Omega$\\
%$\alpha \beta \gamma \delta \epsilon \zeta \eta \theta \iota \kappa \lambda \mu \nu \xi o \pi \rho \sigma \tau \upsilon \phi \chi \psi \omega$



%
% Old hacks
%

% hack for emptyset
% (not needed for mdsymbol)
%\renewcommand{\emptyset}{ {\diameter} }

% make calligraphic bold
%\let\mathcal\mathbcal


==> style/nth.tex <==
% nth.sty  version 2002/27/02 Donald Arseneau
% Ordinal numbering style, 1st 2nd 3rd 4th 5th... 12th... 101st 102nd...
%
% (Public domain: take, include, extract, whatever)
%
% In LaTeX: 
%           \usepackage[super,negative]{nth}
% where option [super] gives superscript `th'
% and option [negative] allows ``st, nd, rd'' suffixes on negative numbers.
%
% example:  \renewcommand{\thesection}{\ordinal{section}}
% or        \renewcommand{\thesection}{\@ordinal\c@section}
% or        \renewcommand{\thesection}{\nth\c@section}
%   
% In plain TeX: 
%           \input nth.sty
% use:      \nth{<number>}.
% Change formatting by redefining \nthscript and \nthtest

% modified to be also able to do things like \nth{i}
% (in this case, always "th" is used)

% ToDo:
% \nth{(n+1)} should give (n+1)^st

\usepackage{xstring}

% optionally specify desired subscript
\DeclareDocumentCommand \nth { m g } % optinal argument in curly braces
{%
    \IfNoValueTF {#2}%
    {%
        \IfInteger{#1}%
        {\nthH{#1}}%
        {{#1\nthscript{th}}}%
    }%
    {%
        {#1\nthscript{#2}}%
    }%
}%


\def\nthH#1{% First print number:
    \expandafter\nthM \number #1\relax
    \nthscript{%
        \ifnum#1\nthtest0 th\else % negatives are all ``th'' (depending on \nthtest)
        \expandafter \nthSuff \expandafter 0\number\ifnum #1<0-\fi#1\delimiter
        \fi
    }}
    
% Minus sign using math mode:
\def\nthM#1{\if -#1\ifmmode-\else$-$\fi\else #1\fi}

% Print suffix depending on last two digits:
\def\nthSuff#1#2#3{%
    \ifx \delimiter#3% #1#2 are last two digits
    \ifnum #1=1 th%  teens are always ``th''
    \else % use appropriate suffix
    \ifcase #2 th\or st\or nd\or rd\else th\fi
    \fi
    \else % continue scanning for last two digits
    \expandafter \nthSuff \expandafter #2\expandafter #3%
    \fi}

% Formatting hook for ordinals (\let\nthscript\textsuperscript)
\def\nthscript#1{\textsuperscript{#1}}% alternate: \def\nthscript#1{$\rm^{#1}$}

% Formatting hook for all negative numbers giving ``th''
\def\nthtest{=}  % alternate: \def\nthtest{>}


==> style/operators.tex <==
% ##################
% OPERATORS
% ##################

%\DeclareMathOperator{\Attr}{Attr}
\DeclareMathOperator{\bin}{bin}


==> style/presentation.tex <==
% #######################
% BEAMER SPECIFIC STUFF
% #######################

% Metropolis theme
% (has to be installed)
\usetheme{metropolis}

% ???
\usepackage{booktabs}
\usepackage[scale=2]{ccicons}

% stuff for tikz
\usepackage{pgfplots}
\usepgfplotslibrary{dateplot}

% absolute positioning of boxes
\usepackage[absolute,overlay]{textpos}

% enumeration
\usepackage{enumerate}

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{decproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/theorems_de.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}      [theorem]     {Theorem}
\newtheorem {corollary}     [theorem]     {Korollar}
\newtheorem {lemma}         [theorem]     {Lemma}
\newtheorem {proposition}   [theorem]     {Proposition}
\newtheorem {remark}        [theorem]     {Bemerkung}
\newtheorem {definition}    [theorem]     {Definition}
\newtheorem {notation}      [theorem]     {Notation}
\newtheorem {example}       [theorem]     {Beispiel}
\newtheorem {exercise}      [theorem]     {Aufgabe}
\newtheorem {algo}          [theorem]     {Algorithm}
\newtheorem {claim}         [theorem]     {Behauptung}
\newtheorem {conjecture}    [theorem]     {Hypothese}
\newtheorem {sources}       [theorem]     {Quellen}
\newtheorem {assumption}    [theorem]     {Annahme}
\newtheorem {fact}          [theorem]     {Fakt}
\newtheorem {question}      [theorem]     {Frage}
\newtheorem {defprop}       [theorem]     {Definition \& Proposition}
\newtheorem {deflemma}      [theorem]     {Definition \& Lemma}
\newtheorem {deftheorem}    [theorem]     {Definition \& Theorem}

\theoremstyle{nonumber} 

\newtheorem* {theorem*}         {Theorem}
\newtheorem* {corollary*}       {Korollar}
\newtheorem* {lemma*}           {Lemma}
\newtheorem* {proposition*}     {Proposition}
\newtheorem* {remark*}          {Bemerkung}
\newtheorem* {definition*}      {Definition}
\newtheorem* {notation*}        {Notation}
\newtheorem* {example*}         {Beispiel}
\newtheorem* {exercise*}        {Aufgabe}
\newtheorem* {algo*}            {Algorithm}
\newtheorem* {claim*}           {Behauptung}
\newtheorem* {conjecture*}      {Hypothese}
\newtheorem* {assumption}       {Annahme}
\newtheorem* {sources*}	        {Quellen}
\newtheorem* {fact*}	        {Fakt}
\newtheorem* {question*}        {Frage}
\newtheorem* {defprop*}         {Definition \& Proposition}
\newtheorem* {deflemma*}        {Definition \& Lemma}
\newtheorem* {deftheorem*}      {Definition \& Theorem}

\theoremstyle{withnumber} 


==> style/theorems_en.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}      [theorem]     {Theorem}
\newtheorem {corollary}     [theorem]     {Corollary}
\newtheorem {lemma}         [theorem]     {Lemma}
\newtheorem {proposition}   [theorem]     {Proposition}
\newtheorem {remark}        [theorem]     {Remark}
\newtheorem {definition}    [theorem]     {Definition}
\newtheorem {notation}      [theorem]     {Notation}
\newtheorem {example}       [theorem]     {Example}
\newtheorem {exercise}      [theorem]     {Exercise}
\newtheorem {algo}          [theorem]     {Algorithm}
\newtheorem {claim}         [theorem]     {Claim}
\newtheorem {conjecture}    [theorem]     {Conjecture}
\newtheorem {assumption}    [theorem]     {Assumption}
\newtheorem {sources}       [theorem]     {Sources}
\newtheorem {fact}          [theorem]     {Fact}
\newtheorem {question}      [theorem]     {Question}
\newtheorem {defprop}       [theorem]     {Definition \& Proposition}
\newtheorem {deflemma}      [theorem]     {Definition \& Lemma}
\newtheorem {deftheorem}    [theorem]     {Definition \& Theorem}

\theoremstyle{nonumber} 

\newtheorem* {theorem*}         {Theorem}
\newtheorem* {corollary*}       {Corollary}
\newtheorem* {lemma*}           {Lemma}
\newtheorem* {proposition*}     {Proposition}
\newtheorem* {remark*}          {Remark}
\newtheorem* {definition*}      {Definition}
\newtheorem* {notation*}        {Notation}
\newtheorem* {example*}         {Example}
\newtheorem* {exercise*}        {Exercise}
\newtheorem* {algo*}            {Algorithm}
\newtheorem* {claim*}           {Claim}
\newtheorem* {conjecture*}      {Conjecture}
\newtheorem* {assumption*}      {Assumption}
\newtheorem* {sources*}	        {Sources}
\newtheorem* {fact*}	        {Fact}
\newtheorem* {question*}        {Question}
\newtheorem* {defprop*}         {Definition \& Proposition}
\newtheorem* {deflemma*}        {Definition \& Lemma}
\newtheorem* {deftheorem*}      {Definition \& Theorem}

\theoremstyle{withnumber} 


==> style/tikz.tex <==
% ########################
% TIKZ
% ########################

% Includes
\usepackage{tikz}
\usepackage{pgf}
\usepackage{tikz-dependency}
\usetikzlibrary{arrows}
\usetikzlibrary{automata}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{petri}
\usetikzlibrary{calc} 
\usetikzlibrary{decorations}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{positioning}
\usetikzlibrary{patterns}
\usetikzlibrary{petri}
\usetikzlibrary{fit}
\usetikzlibrary{graphs} 
\usetikzlibrary{calc}
\usetikzlibrary{tikzmark}

\tikzset{
    treenode/.style = {align=center, inner sep=0pt, text centered,
        font=\sffamily},
    roundpos/.style = {treenode, circle, black, draw=black,
        minimum size=2.5em},
    squarepos/.style = {treenode, rectangle, black, draw=black,
        minimum width=2em, minimum height=2em},
}

\tikzset{
    invisible/.style={opacity=0},
    visible on/.style={alt={#1{}{invisible}}},
    alt/.code args={<#1>#2#3}{%
        \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} % \pgfkeysalso doesn't change the path
    },
}

%
% Transition Boxes
%
\tikzset
{
    tboxoutline/.style = 
    {
        draw,
        thick,
        minimum size=6em,
        inner sep=0pt,
        outer sep=0pt,
    },
    tboxstate/.style =
    {
        minimum width=4pt,
        minimum height=2pt,
        inner sep=0pt,
        fill
    },
    tboxarrow/.style =
    {
    },
    pics/tbox/.style 2 args =
    {
        code =
        {
            \node[tboxoutline,pic actions] (-box) {};
            \foreach \i in {1,...,#1}
            {
                \path
                    (-box.north west)
                    --
                    node
                        [tboxstate,anchor=east,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-in-\i)
                        {}
                    (-box.south west);
                \path
                    (-box.north east) --
                    node
                        [tboxstate,anchor=west,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-out-\i)
                        {}
                (-box.south east);
            }
            
            \foreach \i/\j/\d in {#2}
            {
                \draw
                    [   
                        tboxarrow,
                        decoration =
                        {
                            markings,
                            mark=
                                at position 1 with
                                {
                                    \arrow[scale=1,>=triangle 45]{>}
                                }
                        }
                        ,
                        postaction={decorate}
                    ]
                    (-box-in-\i.east)
                    --
                    node
                        [pos=.8,\d]
                        {}
                    (-box-out-\j.west);
            }
        }
    },
    tbox color/.style={
        tboxstate/.append style={fill=#1},
        tboxoutline/.append style={draw=#1},
        tboxarrow/.append style={draw=#1},
    },
    trans/.style =
    {
        thick,
    },
    dot/.style =
    {
        circle,
        draw,
        minimum size=6pt,
        inner sep=0pt,
        fill,
    },
}

